The ATLAS discovery potential for MSSM neutral Higgs bosons decaying to a mu+mu- pair in the mass range up to 130 GeV

Results are presented on the discovery potential for MSSM neutral Higgs bosons in the Mh-{max}scenario. The region of large tan beta, between 15 and 50, and mass between ~ 95 and 130 GeV is considered in the framework of the ATLAS experiment at the Large Hadron Collider (LHC), for a centre-of-mass energy = 14 TeV. This parameter region is not fully covered by the present data either from LEP or from Tevatron. The h/A bosons, supposed to be very close in mass in that region, are studied in the channel h/A -> mu+mu- accompanied by two b-jets. The study includes a method to control the most copious background, Zo -> mu+mu- accompanied by two b-jets. A possible contribution of the H boson to the signal is also considered.

==> detector.tex <==
\section{Experimental tool: ATLAS detector}


In the following the main features of the ATLAS detector ~\cite{ATLAS01} relevant for the present  analysis are briefly summarized, referring elsewhere
 for a more detailed informations ~\cite[Froidevaux:2006rg] :

\begin{itemize}
\item {\bf Magnet System}:
 The choise of magnet system was  driven by the requirement to achieve a high precision stand-alone momentum measurement of muons over as large acceptance possible.
 It is composed of: a) a solenoid, which provides a 2 T$\cdot$m bending power for the inner detector, b) a barrel air toroid, consisting of eight flat coils of 25m length.
 The bending power for muons is typically 3~T$\cdot$m and c) Two end-cap toroids, which provide a field of  6~T$\cdot$m for muon momentum measurements.
\item {\bf Inner Tracking System}: It has been designed to measure as precise possible and with high efficiency
 the charged particles emerging from primary interactions in a pseudorapidity rage  $\left| \eta \right| < 2.5  $.
 It is installed inside in the solenoid magnetic field and consists of  Si pixels and silicon strip detectors near the interaction point, and strawtubes. 
The expected transverse momentum resolution of the inner tracker for 100 \GeV~ a  charged particle at $\left| \eta \right| =0  $  is $\approx  3.8\%$.
\item {\bf Electromagnetic Calorimeter System} The excellent energy resolution and particle identification for electron, photons and jets demanded from physics is realized
 from a   liquid argon-lead  sampling calorimeter with accordion shape in the barrel and end-cap regions.
% The energy resolution  expected  is for  100 \GeV photon is $1- 1.3 \%$, for 50 \GeV electron is $1.3-1.3 \%$ (trasparenze David)
  The energy resolution in the barrel part of detector can be parametrized as $\frac{\sigma}{\rm{E}}= \sim \frac{10\%}{\sqrt{\rm{ E}}}\oplus 0.2$
 \item {\bf Hadronic Calorimeter}: It is a copper-liquid argon calorimeter  in  the end-cap region  and a Fe-scintillator calorimeter  scintillators in barrel region. 
The liquid argon tungsten forward calorimeters extend the coverage to $\left|\eta \right|$ =4.9.
 The  expected  hadronic jet energy resolution is  $\frac{\sigma}{\rm{E}}=\frac{4.7}{E}\oplus \sim \frac{55\%}{\sqrt{\rm{ E}}}\oplus 0.013$ in the central region. 
\item {\bf Muon spectrometer}. The  reconstruction of muons at highest luminosity is one of the most important point in the ATLAS design.
 The ATLAS toroidal magnet field provides a muon momentum resolution  roughly independent from pseudorapidity using a
  spectrometer  constitued by:
 a) The precision tracking chambers made of 
 Monitored Drift Tubes (MDT) covering the rapidity range $\left| \eta \right| < 2.7  $. b) The Cathode Strip Chambers (CSC) and transverse coordinate strips cover the most forward rapidity region (  $\left|  \eta \right|  = 2.0- 2.7 $) in the  inner most stations of the muon system. c)  Resistive Plate Chambers (RPC) in the barrel region (  $\left| \eta\right|  < 1 $) and  Thin Gap Chambers (TGC) in the end-cap region  provide  muon triggers and measure  the second coordinate of the muon tracks. 
The expected momentum resolution ranges from about 1.4\% for 10 GeV muons to 2.6\% for 100 GeV muons  at$\left| \eta \right| =0  $
\end{itemize}



